Improving the scalabiliy of neutron cross-section lookup codes on multicore NUMA system

We use the XSBench proxy application, a memory-intensive OpenMP program, to explore the source of on-node scalability degradation of a popular Monte Carlo (MC) reactor physics benchmark on non-uniform memory access (NUMA) systems. As background, we present the details of XSBench, a performance abstraction "proxy app" for the full MC simulation, as well as the internal design of the Linux kernel. We explain how the physical memory allocation inside the kernel affects the multicore scalability of XSBench. On a sixteen-core, two-socket NUMA testbed, the scaling efficiency is improved from a nonoptimized 70% to an optimized 95%, and the optimized version consumes 25% less energy than does the nonoptimized version. In addition to the NUMA optimization we evaluate a page-size optimization to XSBench and observe a 1.5x performance improvement, compared with a nonoptimized one.

==> copyright.tex <==
\clearpage 
\onecolumn 
\noindent 
The submitted manuscript has been created by UChicago Argonne, LLC, 
Operator of Argonne National Laboratory (\mbox{``Argonne''}). 
Argonne, a U.S. Department of Energy Office of Science laboratory, is 
operated under Contract No.\ DE-AC02-06CH11357. The U.S. Government 
retains for itself, and others acting on its behalf, a paid-up 
nonexclusive, irrevocable worldwide license in said article to reproduce, 
prepare derivative works, distribute copies to the public, and perform 
publicly and display publicly, by or on behalf of the Government. 

